Re-Search for The Truth: Multi-round Retrieval-augmented Large Language Models are Strong Fake News Detectors

The proliferation of fake news has had far-reaching implications on politics, the economy, and society at large. While Fake news detection methods have been employed to mitigate this issue, they primarily depend on two essential elements: the quality and relevance of the evidence, and the effectiveness of the verdict prediction mechanism. Traditional methods, which often source information from static repositories like Wikipedia, are limited by outdated or incomplete data, particularly for emerging or rare claims. Large Language Models (LLMs), known for their remarkable reasoning and generative capabilities, introduce a new frontier for fake news detection. However, like traditional methods, LLM-based solutions also grapple with the limitations of stale and long-tail knowledge. Additionally, retrieval-enhanced LLMs frequently struggle with issues such as low-quality evidence retrieval and context length constraints. To address these challenges, we introduce a novel, retrieval-augmented LLMs framework--the first of its kind to automatically and strategically extract key evidence from web sources for claim verification. Employing a multi-round retrieval strategy, our framework ensures the acquisition of sufficient, relevant evidence, thereby enhancing performance. Comprehensive experiments across three real-world datasets validate the framework's superiority over existing methods. Importantly, our model not only delivers accurate verdicts but also offers human-readable explanations to improve result interpretability.

==> sections/3_motivation.tex <==
\section{Motivation}

\textbf{Motivation 1: The Internet as a Rich Source of Evidence-Based Information.}
%\wei{what do you mean by saying "valuable"? do you mean "relevant"?}
The Internet is a treasure trove of information, providing a wide array of resources that can enhance individual understanding and viewpoints. While it's true that the Internet is rife with unverified or inaccurate content, credible and factual information remains more prevalent. According to the study ~\cite{DBLP:conf/www/Papadogiannakis23}, despite the existence and occasional popularity of fake news websites, authentic news sources continue to dominate in terms of overall user engagement. 

 
% The Internet is an information-rich reservoir with a plethora of useful and accurate information. In other words, although a large amount of unverified information do exist on the Internet, there is still far more authentic information. 

\textbf{Motivation 2: Advanced Reasoning and Decision-making Capabilities of LLMs.} LLMs have set new records on a variety of Natural Language Inference tasks and demonstrated impressive reasoning capabilities. Although they are not without their flaws—such as challenges in numerical comprehension and a tendency to produce unsupported statements—they consistently surpass traditional machine learning approaches in reasoning and judgment.
As illustrated in Figure \ref{fig:hypo} in Appendix, LLMs possess the unique ability to autonomously decide whether to re-search for additional evidence when the existing information is deemed insufficient. This underscores their potential to adapt and make informed decisions, particularly in tasks requiring evidence-based judgments.

==> tables/ablation_ssm.tex <==
\begin{table}[!hp]
  \centering
  \small
  %\caption{\lgh{Results of the ablation study of semantic search module, the evaluation metric is F1-Ma.}}
  
\begin{tabular}{lccc}
\toprule
\ & \textbf{STEEL} & \textbf{STEEL w/o SSM} \\ \hline
\textbf{LIAR} & \textbf{0.714} & 0.702 \\ \hline
\textbf{CHEF} & \textbf{0.793} & 0.780 \\ \hline
\textbf{POLITIFACT} &	\textbf{0.751} & 0.739   \\ 
\bottomrule
% Weibo & 0.827 & 0.800 & 83.33\%  \\ \hline
\end{tabular}
\caption{Experimental results of the ablation analysis of the semantic search module. The evaluative metric utilized here is F1-Ma.}
  \label{tab:ssm_ablation}
\end{table}

==> tables/difference_with_other_RAG-LLM.tex <==

% \begin{table}[]
%     \centering   
%     \small % 缩小字体 
%     \caption{Comparison of retrieval strategies between STEEL and other methodologies within the RAG+LLM framework.}   
%     \label{tab:difference} 
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{lcccc}
%         \toprule     
%         & \makecell{\textbf{FLARE}\\ \cite{DBLP:conf/emnlp/JiangXGSLDYCN23}} & \makecell{\textbf{Replug} \\ \cite{DBLP:journals/corr/abs-2301-12652}} & \makecell{\textbf{SKR}\\ \cite{DBLP:conf/emnlp/WangLSL23}} & \textbf{STEEL} \\
%          \midrule
%         \textbf{Retrieved Content} & Text chunk & Document & Text chunk & Document or Text chunk \\
%         \textbf{Retrieval Timing} & In-context & In-context & Need more information & Need more information \\
%         \textbf{Information Source} & Wiki & Wiki & Wiki and others & Internet \\
%         \textbf{Retrieval Steps} & $\geq{1}$ & $1$ & $1$ & $\geq{1}$ \\
%         \textbf{Active Search} & Yes & No & Yes & Yes \\
%         \textbf{Utilization of LLM Feedback} & No & No & No & Yes \\
%         \textbf{Answer Verification} & No & No & No & Yes \\    
%         \bottomrule   
%     \end{tabular}
%     }
% \end{table}





% \begin{table}
%   \centering
%   \small % 缩小字体
%   \caption{The difference between STELL and other claims as the query RAG+LLM.}
%   \label{tab:difference}
%   \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|X|X|}
%     \hline
%     & \textbf{What to retrieve} & \textbf{When to retrieve} & \textbf{Retrieve from where} & \textbf{Retrieve times} & \textbf{Whether actively search} & \textbf{Whether to utilize LLM feedback} & \textbf{Check answer} \\
%     \hline
%     \ FLARE~\cite{DBLP:conf/emnlp/JiangXGSLDYCN23} & Text chunk & In-context & Wiki & $\geq{1}$ & Yes & No & No \\
%     \hline
%     \ Replug~\cite{DBLP:journals/corr/abs-2301-12652} & Document & In-context & Wiki & $1$ & No & No & No \\
%     \hline
%     \ SKR~\cite{DBLP:conf/emnlp/WangLSL23} & Text chunk & Need more information & Wiki and others & $1$ & Yes & No & No \\
%     \hline
%     \ STEEL & Document/Text & Need more information & Internet & $\geq{1}$ & Yes & Yes & Yes \\
%     \hline
%   \end{tabularx}
% \end{table}
% \begin{table}[]
%     \centering   
%     %\small % 缩小字体 
%     \caption{Comparison of retrieval strategies between STEEL and other methodologies within the RAG+LLM framework.}   
%     \label{tab:differences} 
%     \resizebox{\textwidth}{!}{
%     \begin{tabular}{cccccccc}
%         \toprule     
%         & \textbf{Retrieved Content} & \textbf{Retrieval Timing} & \textbf{Information Source} & \textbf{Retrievals Times} & \textbf{Active Search} & \textbf{Utilization of LLM Feedback} & \textbf{Answer Verification} \\     
%         \midrule     
%         FLARE~\cite{DBLP:conf/emnlp/JiangXGSLDYCN23} & Text chunk & In-context & Wiki & $\geq{1}$ & Yes & No & No \\     
%         Replug~\cite{DBLP:journals/corr/abs-2301-12652} & Document & In-context & Wiki & $1$ & No & No & No \\     
%         SKR~\cite{DBLP:conf/emnlp/WangLSL23} & Text chunk & Need more information & Wiki and others & $1$ & Yes & No & No \\     
%         STEEL & Document or Text chunk & Need more information & Internet & $\geq{1}$ & Yes & Yes & Yes \\     
%         \bottomrule   
%     \end{tabular}
%     }
% \end{table}

% \begin{table}
%     \centering   
%     \small % 缩小字体   
%     %  \caption{\lgh{The difference between STELL and other claims as the query RAG+LLM}}   \label{tab:difference}  
%     \caption{Comparison of retrieval strategies between STEEL and other methodologies within the RAG+LLM framework.}   \label{tab:difference}  
    
%     \begin{tabularx}{\textwidth}{@{}lX*{6}{X}@{}}     
%         \toprule     
%         & \textbf{Retrieved Content} & \textbf{Retrieval Timing} & \textbf{Information Source} & \textbf{Retrievals Times} & \textbf{Active Search} & \textbf{Utilization of LLM Feedback} & \textbf{Answer Verification} \\     
%         \midrule     
%         FLARE~\cite{DBLP:conf/emnlp/JiangXGSLDYCN23} & Text chunk & In-context & Wiki & $\geq{1}$ & Yes & No & No \\     
%         Replug~\cite{DBLP:journals/corr/abs-2301-12652} & Document & In-context & Wiki & $1$ & No & No & No \\     
%         SKR~\cite{DBLP:conf/emnlp/WangLSL23} & Text chunk & Need more information & Wiki and others & $1$ & Yes & No & No \\     
%         STEEL & Document or Text chunk & Need more information & Internet & $\geq{1}$ & Yes & Yes & Yes \\     
%         \bottomrule   
%     \end{tabularx} 
% \end{table}
